A Multi-Site Accelerator-Rich Processing Fabric for Scalable Brain-Computer Interfacing

Hull is an accelerator-rich distributed implantable Brain-Computer Interface (BCI) that reads biological neurons at data rates that are 2-3 orders of magnitude higher than the prior state of art, while supporting many neuroscientific applications. Prior approaches have restricted brain interfacing to tens of megabits per second in order to meet two constraints necessary for effective operation and safe long-term implantation -- power dissipation under tens of milliwatts and response latencies in the tens of milliseconds. Hull also adheres to these constraints, but is able to interface with the brain at much higher data rates, thereby enabling, for the first time, BCI-driven research on and clinical treatment of brain-wide behaviors and diseases that require reading and stimulating many brain locations. Central to Hull's power efficiency is its realization as a distributed system of BCI nodes with accelerator-rich compute. Hull balances modular system layering with aggressive cross-layer hardware-software co-design to integrate compute, networking, and storage. The result is a lesson in designing networked distributed systems with hardware accelerators from the ground up.

==> tex/conclude.tex <==
\section{Conclusion}
\label{conclude}

==> tex/outline.tex <==
\begin{enumerate}
    \item Introduction
    
    DARPA NESD: The program aims to develop an interface that can read 10$^$6 neurons, write to 10$^$5 neurons, and interact with 10$^$3 neurons full-duplex, a far greater scale than is possible with existing neurotechnology.
    
    \begin{itemize}
        \item IoT systems with high data rates, and extreme environmental constraints are becoming more ubiquitous. \abnote{Explain the nature of constraints and explain how high the data rates are; e.g., AR/VR, autonomous vehicles, smart factories, etc.}
        
        \item Traditionally, these systems have been designed like sensors, without any complicated processing logic or storage at the edge nodes
        
        \item However, recently many domains are adding some logic and storage in these devices to meet the low latency requirements of the applications in these domains
        
        \item This is driven by two key trends: high density, low power storage, and application specific hardware design
        
        \item For these systems to be useful, there needs to be a framework that allows the creation, storage, and analysis of data
        
        \item High-data rates along with the environmental constraints makes the design of storage stacks difficult
        
        \item Brain-Computer Interface (BCI) systems are an extreme design point in the data rates and environmental constraints. This makes creating a data storage stack for BCI systems even harder, and such systems require these storage stacks to be built to help researchers , clinicians, and users improve medical tech (etc)
        
        \item Low power storage storage and application specific hardware design is not enough to design these systems. Consider the following BCI applications that demonstrate this ---

        \begin{itemize}
            \item Seizure graph tracking collects sensor data from multiple sources, detects if a seizure is taking place, if so, calculates correlation between signals from different sources, then treats it if correlation is higher than  threshold (temporary explanation). All this must complete within a tight 5-10 ms constraint
            \item Naively implementing this query in hardware will violate the latency constraint; a design that transmits all data to a single node, even with a perfect hardware that meets the power constraint, will still violate the latency constraint due to transmission latency
            \item This demonstrates such a system requires carefully navigating the design space with a multiple constraint satisfaction problem (satisfy power, latency, bandwidth, each being a tradeoff)
        \end{itemize}

        \item Additionally, due to the extreme constraints in the domain, there is a need to co-design the storage stack to aid the processing stack. 
        
        \begin{itemize}
            \item Consider the spikesorting problem. State-of-the-art algorithms for spikesorting use template matching (explain the range query here).
            \item Spikesorting is an important class of applications that requires extremely low latency. Thus, these queries need high bandwidth access to storage as well as extremely fast filtering access to EEG data
        \end{itemize}
    
        \item The addition of storage to these devices bring a new class of problems that needs to be addressed for satisfactory use of such devices. 
        \begin{itemize}
            \item Due to extreme power conditions, the radio on these devices are extremely limited in their range. As such, these devices frequently drop connections.
            \item It is preferable to analyze all of the data. A storage unit provides excellent opportunity to buffer data as much as possible. However, the storage unit cannot be a persistent store for this data. Eventually, it will fill up, and data must be downloaded or dropped in order to continue recording.
            \item If the device still does not get connectivity, then it will need to discard data to make more space. However, there is debate in the neuroscientific community on which part of the data is interesting for their analysis. 
            \item Thus, a principled approach to data degradation is needed to allow clinicians and neuroscientists access to the most interesting parts of the data at high fidelity, whereas the rest is degraded, or just discarded. 
        \end{itemize}
        
        \item These problems have been explored before in different areas, but not simultaneously. Earlier work that solves a similar problem cannot be retrofit for our needs --- 
            \begin{enumerate}
                \item Distributed databases. Loose argument: Made for datacenters; they navigate the tradeoff on function and data placement to optimize for latency, but don't include power in their calculations.
                \item Prior IoT systems. Loose argument: Typically target lower data rates, looser constraints. Specialized for the application \knote{We specialize as well; need to discuss this point. We allow our system to figure out optimal placement given resources; these typically fix the design after statically finding the a feasible strategy}
                \item Storage devices. Loose argument: they don't target co-designing low power index for time series range queries for nand flashes (the query that our applications need)
            \end{enumerate}
        
        \comments{
            \item BCI systems, as shown in figure 1, can have multiple heterogeneous components that work in tandem to run a BCI application.
            
            \item As a BCI system is used for medical applications, such systems are subject to extreme power, network bandwidth, and latency constraints. 
    
            \item Prior work has looked at optimizing individual components in isolation. Specifically, designs use hardware specialization to meet the extreme constraints imposed on the individual component.
    
            \item However, we show that for BCI applications, it is necessary to optimize the BCI system as a whole to meet power, latency, and network communication constraints.
            
            \item Consider the following applications where a BCI system has to meet multiple constraints ---
            \begin{enumerate}
                \item Movement intent decoding: 
                    \begin{itemize}
                        \item Application where a neural implant is used to decode movement intent to assist a patient with physical therapy.
                        \item System consists of a BCI implant device and a VR device. 
                        \item The implant produces high data rate (~50 Mbps). 
                        \item This data must be processed to find direction of intended movement by user, which is then processed further by the VR device to provide feedback for the therapy.
                        \item The application must be completed within 5-10 ms to deliver effective treatment.
                        \item Transmitting this data over the network incurs transmission delay which is unacceptable for the application.
                        \item However, the implant device is subject to extreme power constraints, reducing the processing that can be pushed on device.
                        \item Thus, we see a trade-off that the system must navigate to find effective plan to run the application such that it can meet all constraints for the application.
                        \item \knote{I need to emphasize the use of storage here. Its not explained at all right now}
                    \end{itemize}
                \item Graph Seizure tracking:
                    \begin{itemize}
                        \item Application where multiple neural implants is used to track seizures through multiple regions of the brain to treat it.
                        \item System consists of a number of neural implants on single patient.
                        \item Each implant produces a high data rate.
                        \item On detection of seizure at an implant, application requires calculating normalized correlations of data between channels of all implants
                        \item This again exposes a tradeoff between communication, latency, and power that a BCI system needs to solve to find a feasible solution
                    \end{itemize}
                \item Interactive analysis:
                    \begin{itemize}
                        \item BCIs used actively both in clinical and research settings to analyze neural data
                        \item User would like to analyze data for interesting events interactively
                        \item Due to network unavailability, most recent data is on device
                        \item Thus, there's a need to increase the throughput of the device to scan for these interesting events and report them at interactive latencies
                        \item \knote{This section needs to be improved. I wasn't sure how to club this need together with the other two, its very specific to single device. It does emphasize the need for storage and local compute}
                    \end{itemize}
            \end{enumerate}

            \item This design space is multi-dimensional, and thus difficult to explore to find a feasible solution. Earlier work that solves a similar problem cannot be retrofit for our needs --- 
                \begin{enumerate}
                    \item Distributed databases. Loose argument: Made for datacenters; they navigate the tradeoff on function and data placement to optimize for latency, but don't include power in their calculations.
                    \item Prior IoT systems. Loose argument: Typically target lower data rates, looser constraints. Specialized for the application \knote{We specialize as well; need to discuss this point. We allow our system to figure out optimal placement given resources; these typically fix the design after statically finding the a feasible strategy}
                    \item Storage devices. Loose argument: they don't target co-designing low power index for time series range queries for nand flashes (the query that our applications need)
                \end{enumerate}
            \item ``What does BrainDump do to solve this?"
                \begin{itemize}
                    \item We note that BCI applications can be expressed with existing relational database abstractions, extended with signal processing routines. We reuse these abstractions.
                    
                    \item Since BCIs are a nascent field, we take this opportunity to co-design our hardware with these known abstractions. This allows us to benefit from simplified programmability for the entire system and get power efficient hardware.
                    
                    \item We express the constraints faced by our BCI system for a particular application as a Linear Programming Problem. We then use an LP solver to find a feasible solution and create a query plan for our application. We note here that by reusing the existing abstractions for databases, expressing the LPP has become easier. \knote{Note: still need to verify its a linear problem. Look at section 3 for part of the equations}
                    
                    \item We co-design the storage stack with NAND flash characteristics to supply the processing stack with high throughput datarates. Specifically, we decide the most cost effective layout to balance the low latency needs of our application while minimizing power used.
                    
                    \item We design a specialized index for NAND flashes to optimize lookups for EEG signals to provide low latency access for some BCI applications. 
                    
                    \item \knote{TODO:: Add explanation for layout design to reduce accuracy when storage is filled } 
                    
                \end{itemize}
                }
            \abnote{End of stuff AB has not looked at}

        
        \item Our contributions: we use hardware-software co-design to implement the following ---
            \begin{itemize}
                \item Query execution plan (Control plane): We study the creation of a physical query plan for a system with inter-device and intra-device heterogeneity along with extreme constraints on power and tight constraint on latency. This will be generally useful as heterogenous devices will be more common for IoT devices in contrained environments.
                We are the first to create an expression of this problem as a Linear Programming problem that can be used more generally to solve this problem in other domains than BCIs
                
                \item Storage Design (Data plane): We design our storage organization and indexes for time series data for low-power NAND flash devices and real-time latencies. The nexus of low power, real-time latency and use of NVMs as physical storage on IoT devices is going to proliferate. Our approach, which is to co-design data structures with the underlying NVM physical hardware to meet real time and power constraints will be applicable to other IoT systems which generate high volumes of time series data, and particularly tend to require higher volumes of reads than writes.
                
                \item Principled data degradation (Data plane): IoT systems generally operate in intermittent connections, that necessitates dropping parts of the data to provide an approximation of the result that an application can tolerate. Prior systems have made use of techniques that allow inferring such properties using extra data structures and computation. Such techniques cannot be afforded in low power IoT settings. We solve this using (the method TBD). This method can be generally applicable to other IoT applications under TBD caveats.
            \end{itemize}
        
        \end{itemize}
    \item Background
        \begin{itemize}
            \item Brain-Computer Interfaces (individual unit)
            \begin{itemize}
                \item Existing compoenents
                \item Constraints placed
            \end{itemize}
            \item BCI systems
                \begin{itemize}
                    \item Explain potential systems that BCIs can be placed in
                    \item Eg: Single implanted BCIs with edge devices, Multiple implanted devices, etc
                \end{itemize}
            \item Nand Flash Memories
                \begin{itemize}
                    \item Read, write characteristics (page granularity). Erase characterisitcs. Plane-parallel reads. Chip parallel ops. 
                \end{itemize}
        \end{itemize}
    \item Motivating BCI applications \knote{Explain motivating examples here in detail with constraints --- see applications in introduction section}
        \begin{itemize}
            \item Multi-device example
            \item Continuous query examples
            \item Analytical query examples
        \end{itemize}
    \item Design Overview
        \begin{itemize}
            \item We go over all components of the system and walkthrough the execution of a query in this section
            \item User creates a query in a familiar language. This includes any additional constraints the user wishes to impose on the system, such as latency.
            \item Query is parsed by BrainDump. The query compiler produces an initial DAG of operators for the query.
            \item BrainDump uses its internal document on available resources to schedule the query on, such as the device power budget, radio cost, etc. TODO: decide all necessary information (eg, will BrainDump query the current resources of the device?)
            \item The Query Planner will compile all these constraints into a linear programming problem, then invoke a solver to find a solution for the problem. TODO: Should this search for optimal plan or just a "good enough"  feasible plan? My first hunch is the latter.
            \item This query plan is then compiled to the platform specific binary to configure the devices in the system.
            \item TODO: Need to also explain specifying initialization of these devices and parameters relevant to that
        \end{itemize}
    \item Design
        \begin{itemize}
            \item Query planner
            \begin{itemize}
                \item Take constraints explained in Background section, and motivating examples section, translate them into useful equations here. Incomplete list follows ---
                \item $P_{device1} = P_{compute1} + P_{NVM1} + P_{Radio1} + ...$
                \item $P_{compute1} = $  (generated from query plan, operators placed in device1, i.e. binary on-off for each operator)
                \item $P_{NVM1}$ generated from approx model of NVM costs, and estimated cardinality (if exact can't be guess) of dataset.
                \item $P_{radio} = E_{perbit} * (num\_bits)$ (num\_bits usually should be exact, but if cannot be guessed, then estimated using dataset cardinality)
                \item And so on for each device. Latencies will be expressed similarly for everything, other than radio (Radio and NVM will have fixed cost estimates)
                \item Finally, the optimizing condition will be limiting the power and latency according to the constraint (So $P_{device1} < 15 mW$ etc)
                \item For all our interesting applications, need to verify if our query plan is a feasible solution even with ``real" issues and delays. \knote{For this reason, it may be more interesting to evaluate with a real-NVM chip. Our use case is exact enough that we should be able to estimate pretty close number}
                \item Above mixes the ``implementation" with ``design". The takeaway in this section should be how we utilized our abstractions to make this expression easier. i.e. The expression of our problem is the contribution, the working for BCIs is the proof. \knote{Need to fix this}
            \end{itemize}    
            \item Storage 
                \begin{itemize}
                    \item Layout
                        \begin{itemize}
                            \item Discuss four possible layouts that we have in mind.
                            \item Associated costs, relative frequency of use
                            \item Chart: X-axis: Number of channels, Y-Axis: Power cost for average operation, Comparison of four layouts for power vs channel count.
                            \item Takeaway: deciding the layout for a particular system using these equations. 
                        \end{itemize}
                    \item Index design
                        \begin{itemize}
                            \item Explain queries that need the index. Specify filter expressions that are relevant for BCI applications (Time based range, and HiWA-based range query)
                            \item For such applications, we need fast access to data For this, we chose the radix-tree index.
                            \item TODO explain modifications that will be needed for NAND flashes. Incomplete List - Batched updates, page-level writes, block-level erases.
                            \item Need to evaluate throughput vs any parameters we use for this index (depth of trees, batch, frequency etc)
                        \end{itemize}
                    \item Accuracy and durability trade-off
                        \begin{itemize}
                            \item \knote{This is still a black-box. Not sure how to do this for Nand flashes}
                            \item Challenges: Nand flashes have a block-erase. I.E., erases will be in the range of 1 MB. Getting all of this data out in RAM will consume too much power. Also, random access writes are unavailable in nand flashes. 
                            \item The above indicates a solution potentially lying in an interesting encoding or using a intermediate swap space to store lower fidelity data.
                        \end{itemize}
                \end{itemize}
        \end{itemize}
    \item Methodology and evaluation
        \begin{itemize}
            \item \knote{TODO:: add details of system we test}
        \end{itemize}
    \item Conclusion \& Related Work 
    
\end{enumerate}

==> tex/tab_device.tex <==
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
Capability        & Aziz et al         & Medtronic Activa RC+S         & External(?)     & HALO         & BrainDump        \\ \midrule
Max data rate     & $\sim$50Mbps & $\sim$16Kbps         & $\sim$50Mbps & $\sim$50Mbps & $\sim$50Mbps     \\
Programmable      & No           & Yes                  & Yes          & Yes          & Yes              \\
Scalable accuracy & No           & Yes                  & Yes          & No           & Yes              \\
Storage capacity  & Stream       & $\sim$1.5hrs, Stream & Stream       & Stream       & 24 hours, stream \\
Safety            & Yes          & Yes                  & No           & Yes          & Yes              \\ \bottomrule
\end{tabular}%
}
\caption{Summary of existing systems and BrainDump. \knote{Need to somehow add data,function colocation.}}
\label{tab:device-list}
\end{table}

\begin{comment}
\begin{table}
\centering
\resizebox{\linewidth}{!}{%
    \LARGE{
        \begin{tabular}{@{}lcccccccc@{}}
        \toprule
         & {\LARGE Medtronic} & {\LARGE Neuropace} & {\LARGE Aziz} & {\LARGE Chen} & {\LARGE Kassiri} & {\LARGE Neuralink} & {\LARGE NURIP} & {\LARGE \textbf{\red{HALO}}} \\
         & {\cite{medtronic:manual}} & {\cite{neuropace:rns}} & {\cite{aziz:256:delta}} & {\cite{chen:hardware}} & {\cite{kassiri:closed}} & {\cite{musk:integrated}} & {\cite{leary:nurip}} \\  \midrule
        {\LARGE Computational Pipeline} &  &  &  &  &  &  &  & \\ \midrule
        {\LARGE Spike Detection} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes}  & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\red{\checkmark}}\\
        {\LARGE Compression} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes}  & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes}  & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\red{\checkmark}}\\
        {\LARGE Seizure Prediction} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\checkmark}& \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\checkmark}& \multicolumn{1}{c}{\checkmark}& \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\red{\checkmark}}\\
        {\LARGE Movement Intent} & \multicolumn{1}{c}{\checkmark}& \multicolumn{1}{c}{\texttimes}  & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes}  & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\red{\checkmark}}\\
        {\LARGE Encryption} & \multicolumn{1}{c}{\texttimes} &  \multicolumn{1}{c}{\texttimes}  & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes}  & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\red{\checkmark}}\\ \midrule
        {\LARGE Technical Capabilities}  \\ \midrule
        {\LARGE Programmable} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{Limited} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{Limited} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{Limited} & \multicolumn{1}{c}{\LARGE \red{\checkmark}} \\
        {\LARGE Read Channels} & \multicolumn{1}{c}{\LARGE 4} & \multicolumn{1}{c}{\LARGE 8} & \multicolumn{1}{c}{\LARGE 256} & \multicolumn{1}{c}{\LARGE 4} & \multicolumn{1}{c}{\LARGE 24} & \multicolumn{1}{c}{\LARGE 3072} & \multicolumn{1}{c}{\LARGE 32} & \multicolumn{1}{c}{\LARGE \red{96}} \\
        {\LARGE Storage Capability} & \multicolumn{1}{c}{\LARGE Stream} & \multicolumn{1}{c}{\LARGE \textasciitilde 0.5MB} & \multicolumn{1}{c}{\LARGE Stream} & \multicolumn{1}{c}{\LARGE Stream} & \multicolumn{1}{c}{\LARGE Stream} & \multicolumn{1}{c}{\LARGE ---} & \multicolumn{1}{c}{\LARGE Stream} &  \multicolumn{1}{c}{\LARGE \red{Stream}} \\
        {\LARGE Sample Frequency (Hz)} & \multicolumn{1}{c}{\LARGE 250} & \multicolumn{1}{c}{\LARGE 250} & \multicolumn{1}{c}{\LARGE 5K} & \multicolumn{1}{c}{\LARGE 200} & \multicolumn{1}{c}{\LARGE 7.2K} & \multicolumn{1}{c}{\LARGE 18.6K} & \multicolumn{1}{c}{\LARGE 256} & \multicolumn{1}{c}{\LARGE \red{30K}} \\
        {\LARGE Sample Resolution (bits)} & \multicolumn{1}{c}{\LARGE 10} & \multicolumn{1}{c}{\LARGE 10} & \multicolumn{1}{c}{\LARGE 8} & \multicolumn{1}{c}{\LARGE 10} & \multicolumn{1}{c}{\LARGE -} & \multicolumn{1}{c}{\LARGE 10} & \multicolumn{1}{c}{\LARGE 16} & \multicolumn{1}{c}{\LARGE \red{16}} \\
        %Processor type & FPGA & N/R & VLSI & FPGA & DSP & N/A & HRA \\
        {\LARGE Safety ($<$15mW)} & \multicolumn{1}{c}{\LARGE \checkmark} & \multicolumn{1}{c}{\LARGE \checkmark} & \multicolumn{1}{c}{\checkmark}& \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\checkmark}& \multicolumn{1}{c}{\texttimes} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\red{\checkmark}}\\ \midrule
        \end{tabular}%
    }
}
\caption{\knote{Should HALO be in this list? How best to add prior work? By addressing the fact that HALO only had computational pipelines, not storage?}\knote{The storage capability looks cherry picked; should find more storage BCI devices}}
\label{tab:device-summary}
\end{table}
\end{comment}


==> tex/tables/applications.tex <==
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lrrrr@{}}
\toprule
Application name                   & \multicolumn{1}{l}{Seizure Det} & \multicolumn{1}{l}{Hash} & \multicolumn{1}{l}{DTW} & \multicolumn{1}{l}{Max channels} \\ \midrule
Local Seizure Detection            & 1                               & 0                        & 0                       & 120                              \\
Functional Connectivity Estimation & 0                               & 1                        & 0                       & 182                              \\
Hub similarity                     & 0                               & 0                        & 1                       & 15                               \\
Seizure Propagation                & 1                               & 1                        & 1                       & 96                               \\
Movement Intent                    & NA                              & 1                        & 1                       & 220                              \\
\bottomrule
\end{tabular}%
}
\caption{Table of Applications that Beacon supports}
\end{table}
